Thermometry in Near-Degenerate Nitrogen-Vacancy Ensembles Enabled by Bright-Dark-State Mixing

Nitrogen-vacancy (NV) centers have emerged as a highly sensitive platform for spatially resolved temperature measurements. When the $\lvert0\rangle\to\lvert+1\rangle$ and $\lvert0\rangle\to\lvert-1\rangle$ transitions are nearly degenerate and the Rabi frequency is comparable to the transition splitting, the spin dynamics encountered during pulsed protocols for temperature measurement can significantly alter the intended accumulation of temperature-dependent phase. We investigate these triplet ($\lvert0\rangle$, $\lvert\pm1\rangle$) spin dynamics and their effect on pulsed thermometry protocols under these conditions. We find that the conventional thermal-echo timing produces negligible temperature-sensitive signal amplitudes at the common-mode detuning. However, we find that the nominal spin-echo timing produces resolvable oscillations at the common-mode detuning, leading to a strong temperature-sensitive carrier signal. This departure from the expected protocol behavior is qualitatively captured by an ensemble model of the triplet dynamics, which supports significant dark-state leakage as a plausible mechanism for the temperature-sensitive response. This mixing-enabled thermal echo uses a four-phase quadrature readout that resolves the signed oscillation frequency and is validated using independent sweeps of the microwave carrier frequency and fluid temperature. We further assess the ability of a four-refocusing-pulse (LDD4B) low-field dynamical-decoupling sequence to extend the NV coherence and find that while the echo retains a sensitivity to common-mode detuning, the effective phase-accumulation interval corresponds to approximately half the total evolution time. These findings could support the use of pulsed NV thermometry in biological or mobile applications where applying magnetic bias fields is impractical and microwave power may be limited.

==> figures/data/Figure3a_physical_fit.tex <==
\def\odmrPhysicalBaseline{1.00160414}
\def\odmrPhysicalSlopePerMHz{0.0000009880}
\def\odmrPhysicalDepth{0.02276332}
\def\odmrPhysicalMeanFrequencyMHz{2870.50000}
\def\odmrPhysicalMinFrequencyMHz{2862.50000}
\def\odmrPhysicalMaxFrequencyMHz{2878.50000}
\def\odmrPhysicalCenterGHz{2.87057791}
\def\odmrPhysicalCenterMHz{2870.57791}
\def\odmrPhysicalCenterDetuningMHz{0.078}
\def\odmrEffectiveStrainMHz{0.58125}
\def\odmrEffectiveStrainCiLowMHz{0.27211}
\def\odmrEffectiveStrainCiHighMHz{0.89039}
\def\odmrPhysicalHwhmMHz{0.76001}
\def\odmrPhysicalFwhmMHz{1.52002}
\def\odmrPhysicalMinBranchMHz{2867.19173}
\def\odmrPhysicalMaxBranchMHz{2873.96410}
\def\odmrPhysicalRmsPercent{0.17764}
\def\odmrPhysicalFitRSquared{0.698402}
\def\odmrPhysicalAicc{-1900.03}
\def\odmrPhysicalBranchCount{24}
\def\odmrPhysicalN{151}
\def\odmrPhysicalK{6}
\def\odmrPhysicalReportedMinFrequencyMHz{2862.5}
\def\odmrPhysicalReportedMaxFrequencyMHz{2878.5}
\def\odmrPhysicalReportedMeanFrequencyMHz{2870.5}
\def\odmrPhysicalReportedBaseline{1.0016}
\def\odmrPhysicalReportedSlopePerMHz{0.000001}
\def\odmrPhysicalReportedDepth{0.0228}
\def\odmrPhysicalReportedCenterMHz{2870.58}
\def\odmrEffectiveStrainReportedMHz{0.58}
\def\odmrEffectiveStrainReportedCiLowMHz{0.27}
\def\odmrEffectiveStrainReportedCiHighMHz{0.89}
\def\odmrPhysicalReportedHwhmMHz{0.76}
\def\odmrPhysicalReportedMinBranchMHz{2867.19}
\def\odmrPhysicalReportedMaxBranchMHz{2873.96}
\def\odmrPhysicalReportedRmsPercent{0.178}
\def\odmrPhysicalReportedFitRSquared{0.698}
\def\odmrPhysicalReportedAicc{-1900.03}


==> figures/data/Figure3a_two_lobe_fit.tex <==
\def\odmrTwoLobeBaseline{1.00216345}
\def\odmrTwoLobeSlopePerMHz{0.0000000000}
\def\odmrTwoLobeLowerAmplitude{0.00685128}
\def\odmrTwoLobeUpperAmplitude{0.00685128}
\def\odmrTwoLobeMeanFrequencyMHz{2870.50000}
\def\odmrTwoLobeCenterMHz{2870.53981}
\def\odmrTwoLobeHalfSplittingMHz{1.77500}
\def\odmrTwoLobeHalfSplittingCiLowMHz{1.60351}
\def\odmrTwoLobeHalfSplittingCiHighMHz{1.94649}
\def\odmrTwoLobeLowerCenterMHz{2868.76481}
\def\odmrTwoLobeUpperCenterMHz{2872.31481}
\def\odmrTwoLobeLowerDetuningMHz{-1.73519}
\def\odmrTwoLobeUpperDetuningMHz{1.81481}
\def\odmrTwoLobeLowerHwhmMHz{1.60040}
\def\odmrTwoLobeUpperHwhmMHz{1.60040}
\def\odmrTwoLobeRmsPercent{0.17809}
\def\odmrTwoLobeFitRSquared{0.696887}
\def\odmrTwoLobeAicc{-1901.44}
\def\odmrTwoLobeN{151}
\def\odmrTwoLobeK{5}
\def\odmrTwoLobeCommonAmplitude{0.00685128}
\def\odmrTwoLobeCommonHwhmMHz{1.60040}
\def\odmrTwoLobeReportedMinFrequencyMHz{2862.5}
\def\odmrTwoLobeReportedMaxFrequencyMHz{2878.5}
\def\odmrTwoLobeReportedMeanFrequencyMHz{2870.5}
\def\odmrTwoLobeReportedBaseline{1.0022}
\def\odmrTwoLobeReportedSlopePerMHz{0.000000}
\def\odmrTwoLobeReportedLowerAmplitude{0.0069}
\def\odmrTwoLobeReportedUpperAmplitude{0.0069}
\def\odmrTwoLobeReportedCenterMHz{2870.54}
\def\odmrTwoLobeReportedHalfSplittingMHz{1.78}
\def\odmrTwoLobeReportedHalfSplittingCiLowMHz{1.60}
\def\odmrTwoLobeReportedHalfSplittingCiHighMHz{1.95}
\def\odmrTwoLobeReportedLowerCenterMHz{2868.76}
\def\odmrTwoLobeReportedUpperCenterMHz{2872.31}
\def\odmrTwoLobeReportedLowerHwhmMHz{1.60}
\def\odmrTwoLobeReportedUpperHwhmMHz{1.60}
\def\odmrTwoLobeReportedRmsPercent{0.178}
\def\odmrTwoLobeReportedFitRSquared{0.697}
\def\odmrTwoLobeReportedAicc{-1901.44}
\def\odmrTwoLobeReportedCommonAmplitude{0.0069}
\def\odmrTwoLobeReportedCommonHwhmMHz{1.60}
\def\odmrMovingMeanWindow{5}
\def\odmrCenterGHz{2.87054}
\def\odmrCenterMHz{2870.54}
\def\odmrCenterCiLowMHz{2870.34}
\def\odmrCenterCiHighMHz{2870.74}
\def\odmrLowerResonanceMHz{2868.76}
\def\odmrUpperResonanceMHz{2872.31}
\def\odmrDoubletSeparationMHz{3.55}
\def\odmrFitRSquared{0.697}


==> figures/data/Figure3b.tex <==
\def\rabiFitMHz{2.01}
\def\rabiPiOverTwoUs{0.124494}
\def\rabiPiUs{0.248988}
\def\rabiTwoPiUs{0.497977}
\def\rabiPiOverTwoNs{124}
\def\rabiPiNs{249}
\def\rabiTwoPiNs{498}
\def\rabiFundamentalPhaseDeg{180}
\def\rabiSecondHarmonicPhaseDeg{-98.1}

